A New Class of Private Chi-Square Tests

In this paper, we develop new test statistics for private hypothesis testing. These statistics are designed specifically so that their asymptotic distributions, after accounting for noise added for privacy concerns, match the asymptotics of the classical (non-private) chi-square tests for testing if the multinomial data parameters lie in lower dimensional manifolds (examples include goodness of fit and independence testing). Empirically, these new test statistics outperform prior work, which focused on noisy versions of existing statistics.

==> Lap_GOF.tex <==
\subsection{MC Approach for Arbitrary Noise Distributions \label{sect:DP_GOF}}

We now show that we can use both the unprojected and projected statistics in \eqref{eq:simple_stat1} and \eqref{eq:simple_stat2}, respectively, when we instead add other types of noise to the histogram data $\XX{n}$.  We focus on Laplace noise in this section so that our resulting test will ensure differential privacy (DP).  In this case, we apply the Laplace Mechanism from \eqref{eq:LM}  to each cell count by adding independent Laplace noise with scale $2/\epsilon$ to obtain $\epsilon$-DP.  As $1/\rho$ represents the variance of the noise that is added to the cell counts, we replace $1/\rho$ in \eqref{eq:simple_stat1} and \eqref{eq:simple_stat2} with the variance of the additional Laplace noise terms, which is $2/\epsilon^2$.  

\begin{algorithm}
\caption{DP Chi-Squared Goodness of Fit Test using MC}
\label{alg:gof_DP}
\begin{algorithmic}
\Procedure{$\texttt{DP-MC-GOF}$}{Histogram data $X^{(n)} = (X_1^{(n)},\cdots, X_d^{(n)})$; $\epsilon$, $\alpha$, $H_0: \bp = \bp^0$, $m$}
\State Compute either $\QQ{n}_{\epsilon^2/2}$ from \eqref{eq:simple_stat1} or $\hQQ{n}_{\epsilon^2/2}$ from \eqref{eq:simple_stat2} after adding $\Lap(2/\epsilon)$ to each entry of $X$.
\State Set $\{q_1,\cdots, q_m\}$ as $m$ independent samples from the distribution of either $\QQ{n}_{\epsilon^2/2}$ or $\hQQ{n}_{\epsilon^2/2}$.
\State Set $\tau(\alpha,\epsilon)$ to be the $\lceil (m+1)(1-\alpha) \rceil$-largest value of $\{q_1,\cdots, q_m\}$.
\If{$ \QQ{n}_{\rho} > \tau(\alpha,\epsilon)$ or $ \hQQ{n}_{\rho} > \tau(\alpha,\epsilon)$}
\State Decision $\gets$ Reject
\Else
\State Decision $\gets $ Fail to Reject
\EndIf
\State {\bf return} Decision.
\EndProcedure
\end{algorithmic}
\end{algorithm}

Based on the noisy histogram counts $\XX{n} + Z$, we then use either the unprojected statistic in \eqref{eq:simple_stat1} or the projected statistic in \eqref{eq:simple_stat2}.  Unfortunately, in this case the resulting asymptotic distribution is not a chi-squared distribution, due to the additional noise being Laplace rather than Gaussian.  We then rely on Monte Carlo (MC) sampling to determine whether the null hypothesis should be rejected.  



